HiFrames: High Performance Data Frames in a Scripting Language

Data frames in scripting languages are essential abstractions for processing structured data. However, existing data frame solutions are either not distributed (e.g., Pandas in Python) and therefore have limited scalability, or they are not tightly integrated with array computations (e.g., Spark SQL). This paper proposes a novel compiler-based approach where we integrate data frames into the High Performance Analytics Toolkit (HPAT) to build HiFrames. It provides expressive and flexible data frame APIs which are tightly integrated with array operations. HiFrames then automatically parallelizes and compiles relational operations along with other array computations in end-to-end data analytics programs, and generates efficient MPI/C++ code. We demonstrate that HiFrames is significantly faster than alternatives such as Spark SQL on clusters, without forcing the programmer to switch to embedded SQL for part of the program. HiFrames is 3.6x to 70x faster than Spark SQL for basic relational operations, and can be up to 20,000x faster for advanced analytics operations, such as weighted moving averages (WMA), that the map-reduce paradigm cannot handle effectively. HiFrames is also 5x faster than Spark SQL for TPCx-BB Q26 on 64 nodes of Cori supercomputer.

==> discussion.tex <==
\textbf{Running legacy SQL query code:} In order to run the legacy SQL
query code on top of HPAT parallel processing framework, we just need
to write SQL to \hpat{} \df{} parser. As \hpat{} \df{} API has one
to one mapping from \sql{} relational operators, the parser will
essentially translate each SQL operator in the query to corresponding
\hpat{} \df{} API internal representation to generate AST. Once the
AST is generated it will behave in the same way as the query was
written in HPAT's \df{}. We plan to add this parser in the next
release of HPAT \df{}.


==> pattern-match.tex <==
\begin{algorithm}
  \caption{Matching Optimizer rules}\label{algo:pattern}
  %% \begin{algorithmic}[1]
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  \Input{Execution plan tree $tree$, Rule set $rules$}
  \Output{Optimized execution plan tree $optTree$}
  
  \lForEach{node $n$ of the $tree$}{
    
  }
  %% \end{algorithmic}
\end{algorithm}

